BEAR: Physics-Principled Building Environment for Control and Reinforcement Learning

Recent advancements in reinforcement learning algorithms have opened doors for researchers to operate and optimize building energy management systems autonomously. However, the lack of an easily configurable building dynamical model and energy management task simulation and evaluation platform has arguably slowed the progress in developing advanced and dedicated reinforcement learning (RL) and control algorithms for building operation tasks. Here we propose "BEAR", a physics-principled Building Environment for Control And Reinforcement Learning. The platform allows researchers to benchmark both model-based and model-free controllers using a broad collection of standard building models in Python without co-simulation using external building simulators. In this paper, we discuss the design of this platform and compare it with other existing building simulation frameworks. We demonstrate the compatibility and performance of BEAR with different controllers, including both model predictive control (MPC) and several state-of-the-art RL methods with two case studies.

==> environment.tex <==
BEAR enjoys flexibility and high fidelity provided by a variety of user-defined variables as inputs~(see details in Appendix C) and provides an OpenAI Gym interface. Users can perform simulations in the customized environment with any classic model-based control or learning-based controllers. A sample usage of BEAR package in Python is also illustrated in Appendix D.

\textbf{State Space}: The state $s_k$ is the RL agent's observation from a building environment at timestep $k$. It is different from the state space model \eqref{eq:discrete_building_model} by including both $x[k]$ and the uncontrollable inputs observed from the environment. The state space is bounded by user-defined minimum and maximum values. The state $s_k$ is constructed as:
%\begin{equation}s_t=\{\{T_1,T_2...,T_{n}\}_t,\{Q_p\}_t,\{T_G\}_t,\{T_{out}\}_t,\{Q_{ghi}\}_t\}
%\end{equation},
\begin{equation}s_k=[T_1[k],T_2[k], ...,T_{M}[k],Q_p[k],T_G[k],T_{E}[k],Q_{ghi}[k]],
\end{equation}
%Recall that $Q_p$ and $Q_{ghi}$ are the heat generation per person and heat absorbed from global horizontal radiance; $T_G$ and $T_E$ are the ground and outdoor temperature.

\textbf{Action space}: 
The action $a_k$ is generated by the controller given state $s_k$. 
The action $a_k$ is a set of controllable actions constructed with the energy supply of the HVAC system, as shown below:
\begin{equation}
a_k=[Q^z_{1}[k],Q^z_{2}[k],...,Q^z_{M}[k]],
\end{equation}
% The set $a_k^{env}$ is a set of all ``environmental action'' determined by the environment which are uncontrollable,
% \begin{equation}
% a_k^{env}=[].
% \end{equation}
The whole action space is constrained by the maximum HVAC power consumption and normalized within the box of [-1, 1] in the user interface. All actions are rescaled to their original values inside the BEAR simulation. Once an action is selected, the $env.step()$ function provided by OpenAI Gym will take both $s_k$ and $a_k$ as input, and simulate the next state $s_{k+1}$ using BEAR. 

\begin{figure}[t]
\centering
\includegraphics[width=0.35\textwidth]{rp21j.png}
\caption{\label{fig:rp18b} Simulated building examples.\vspace{-10pt}}
\end{figure}

\textbf{Reward}:
A main objective of building control is to reduce the energy consumption while keeping the temperature within given comfort range. %Therefore, the reward function should penalize both temperature violations and high HVAC energy consumption actions. 
Our platform allows users to customize reward function using environment states $s_k$, actions $a_k$, target values $obj_k$ and a weight term $\beta$. We denote such reward function as 
$Reward = R(s_k,a_k,obj_k,\beta)$.
BEAR users can customize reward by changing the weighting term, with small $\beta$ leading to low energy consumption and large $\beta$ leading to small temperature range deviation. One default reward function is the \emph{L2} reward, defined as $$R_k=-(1-\beta)||a_k||_2-\beta||s^{obj}_k-s_k||_2$$ where $s^{obj}_k=[T^{obj}_{1}[k],...,T^{obj}_{M}[k]]$ are the target temperature from user input.
%the reward is defined as $R_k=-(1-\beta)||a_k||_2-\beta||s^{obj}_k-s_k||_2$. 
%as follows:
% \begin{itemize}[leftmargin=*]
%     \item \emph{L2} reward: With target temperature $s^{obj}_k=[T^{obj}_{1}[k],...,T^{obj}_{M}[k]]$ from user input, the reward is defined as $R_k=-(1-\beta)||a_k||_2-\beta||s^{obj}_k-s_k||_2$. 
%     % \item \emph{Exponential} reward: To further avoid extreme temperature or control actions, one can use reward: $R_k=-(1-\beta)Exp(||a_k||_2)-\beta(Exp(||s^{obj.up}_k-s_k||_2+||s^{obj.lo}_k-s_k||_2))$, where $s^{obj.up}_k, \, s^{obj.lo}_k$ denote the upper and lower bound of temperature range.
% \end{itemize}

% \subsubsection{L1 reward}
% \begin{equation}
% R_t=-||[T^{target}_{1},T^{target}_{2},...,T^{target}_{M}]_t-[T_1,T_2...,T_{M}]_t||_1
% \end{equation}
% The above function defines the current timestep reward $R_t$ as the L1 norm of the difference between the current zone temperatures and the target temperatures $T^{target}$. The goal of this reward function is to control the indoor temperature at the target setpoint schedule.



% \begin{equation}
% R_t=-\alpha||a_t||_2-\beta||[T^{target}_{1},T^{target}_{2},...,T^{target}_{M}]_t-[T_1,T_2...,T_{M}]_t||_2
% \end{equation}

%The above function defines the current timestep reward $R_t$ as the negative sum of  the exponential of the absolute energy consumption $a_t$ and the exponential of the total deviation between the current zone temperatures $s_t$ and both the upper bound objective temperatures and lower bound objective temperatures. The minimum total deviation is the  comfort range $s^{obj.upper}_t-s^{obj.lower}_t$.

==> simulation.tex <==
In this section, we demonstrate the usage of BEAR with two building examples. We compare our simulator with EnergyPlus on a rectangular single-story building to validate the fidelity of our simulations. We also compare the performance of different control strategies, including rule-based controller, MPC (which knows the exact building dynamics model), and two RL controllers SAC~\cite{haarnoja2018soft}, PPO~\cite{schulman2017proximal} (which do not assume any model knowledge) on a simulated medium office building. Since our goal is to show the compatibility of our platform with multiple controllers, we directly set up all RL algorithms using Stable-Baselines 3~\cite{stb3}. Detailed variable settings and building type examples can be found in our anonymous code repository.

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{example1noaction.PNG}
\caption{\label{fig:SvA}Comparison of zonal temperature using BEAR simulator and EnergyPlus on the same test building located in Chicago, IL.\vspace{-10pt}}
\end{figure}

\textbf{Single-Story Building}:  
%EnergyPlus is one of the most well-known and authoritative platform for virtual environment simulation of building HVAC system. 
To illustrate the fidelity of our simulator, we first set up a test example building model described in the EnergyPlus documentation and benchmark it against BEAR's simulations. %Five occupied zones compose the single-story structure, and a ceiling plenum is on top of all zones; 
See Fig \ref{fig:rp18b} (A) for the building illustration. Specifically, we set up the physics-based model with building parameters estimated through information provided in the EnergyPlus. We also fit a data-driven model with data simulated by the EnergyPlus. A comparison of the zonal temperature simulated in BEAR and EnergyPlus without any HVAC control is shown in Fig \ref{fig:SvA}. We could see both physics-based and data-driven simulation engine demonstrate good fidelity compared to EnergyPlus. Then, we set the indoor temperature at $22^\circ$C with a daily operating schedule of 8 a.m. to 3 p.m. In Fig \ref{fig:south}, we compare the south zone temperature between our simulator and EnergyPlus using the same control input actions. We also compare the power demand by controlling each zone in the building strictly at the same target temperature. As is shown in Fig \ref{fig:paper2}, under the same operational goal, we validate that not only the daily temperature in both simulations exhibit the same patterns (left), but the energy consumption profile of BEAR also closely tracks EnergyPlus's simulated trajectory (right).
% Specifically, we compare power demand and zonal temperature between our simulator and EnergyPlus by controlling each zone in the building strictly at the same target temperature. We set the indoor temperature at $22^\circ$C with a daily operating schedule of 8 a.m. to 3 p.m. %and run through a whole-year simulation.
% As is shown in Fig \ref{fig:SvA}, under the same control logic, BEAR exhibits nearly the same temperature behaviors for both zones as EnergyPlus. %validating that our physical model is exhibiting realistic building dynamics. 
% In Fig \ref{fig:paper2}, we validate that not only the daily temperature in both simulations exhibits the same patterns (left), but the energy consumption profile of BEAR also closely tracks EnergyPlus's simulated trajectory (right). 





%In this building, each occupied zone is designed to have a unitary HVAC object with electric coils \textcolor{red}{What is unitary object? What is electric coil?}. 
\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{south_epaction.PNG}
\caption{\label{fig:south} Temperature profile comparison with same control.\vspace{-10pt}}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{a6.PNG}
\caption{\label{fig:paper2} Comparison of energy consumption. \vspace{-10pt} }
\end{figure}

\begin{scriptsize}
\begin{table}[t]
\centering
\begin{tabular}{l||p{1.7cm}|p{1.7cm}|p{1.3cm}}
\hline
Controller & Average Temperature Variation($^\circ$C) & Average Daily Energy Consumption (J)& Computation Time (s)\\\hline
Rule-Based Controller&2.537  &1.490E6&0.698 \\\hline
% MPC($\beta=0.99$)&5.1296E-13 &6.257E5 &33.572\\\hline
% MPC($\beta=0.01$)&6.709 &5.616E-6 &33.633\\\hline

MPC ($\beta=0.8$)&2.701E-11 &6.25E5 &33.572\\\hline
PPO ($\beta=0.8$) &0.969 & 6.504E5&1.309  \\\hline
SAC ($\beta=0.8$) &0.795 & 6.188E5&1.348 \\\hline
MPC ($\beta=0.45$)&0.383 &5.87E5 &33.633\\\hline
PPO ($\beta=0.45$) &2.645 & 4.680E5&1.339 \\\hline
SAC ($\beta=0.45$) &1.360 & 5.691E5&1.235 \\\hline
\end{tabular}
\caption{\label{tab:perform}Performance on medium office. \vspace{-15pt}}
\end{table}
\end{scriptsize}

\textbf{Medium Office Building}: 
We also test a medium office building provided by the reference commercial buildings list of the U.S. Department of Energy~\cite{deru2011us}. The building has three stories; each is divided into four perimeter zones, one core zone, and one plenum zone, see Fig \ref{fig:rp18b} (B). 
% \begin{figure}
% \centering
% \includegraphics[width=0.5\textwidth]{rp19g.png}
% \caption{\label{fig:rp19g}OfficeMedium at Tucson.}
% \end{figure}
The HVAC system is operated at all perimeter zones, and we set the indoor temperature of the perimeter zones at $22^\circ$C. We set the location of the building in Tucson, Arizona, and use the weather file of 2003 from January to April for simulation. 
The control agents we tested include a rule-based controller, a MPC, and two RL controllers, namely PPO and SAC. The rule-based controller performs heating when the indoor temperature is below the target setpoint and performs cooling when the temperature is above the setpoint. The MPC, PPO, and SAC controllers are tested with two $L_2$ reward functions with $\beta=0.8$ and $\beta=0.45$ respectively. %One is set with an objective of minimizing the reward with a $\beta=0.8$ weight, meaning it would focus more on approaching the setpoint temperature than reducing the energy consumption. Another minimizes the reward with a $\beta=0.45$ weight on the temperature variation and $1-\beta=0.55$ weight on the sum of action. 
%We also test PPO and SAC agents with the same two reward functions. 
The learning curves of the RL controllers are shown in Appendix A in Fig \ref{fig:trainreward}. We could see that all the RL training rewards are converging, and algorithms with the same reward function converge to a similar objective value. The performance of tested controllers is shown in Table~\ref{tab:perform}. With the implementation of RL algorithms, we can observe that the energy consumption decreases significantly compared to the simple rule-based controller. It also reduces the average temperature variation. Compared to the MPC method, which has complete model knowledge, both model-free RL algorithms obtain a similar or lower energy consumption, with higher temperature violation. The computation time using PPO and SAC is greatly reduced compared to MPC, as the latter needs to solve an optimization problem at each step to obtain action.

% \begin{figure}
% \centering
% \includegraphics[width=0.25\textwidth]{trainingreward.PNG}
% \caption{\label{fig:trainreward}Reward during Training for RL policies.\vspace{-10pt} }
% \end{figure}










